A Benign Activity Extraction Method for Malignant Activity Identification using Data Provenance

In order to understand the overall picture of cyber attacks and to identify the source of cyber attacks, a method to identify malicious activities by automatically creating a graph that ties together the dependencies of a series of related events by tracking Data Provenance has been developed. However, the problem of dependency explosion, in which a large number of normal computer system operations such as operations by authorized users are included in the dependencies, results in a huge generated graph, making it difficult to identify malicious activities. In this paper, we propose a method to reduce the search space for malicious activities by extracting and removing frequently occurring benign activities through natural language processing of log data and analysis of activities in the computer system using similarity judgments. In the evaluation experiment, we used the DARPA TC Dateset, a large-scale public dataset, to evaluate the effectiveness of the proposed method on the dependency explosion problem. In addition, we showed that about 6.8 to 39% of the activities in a computer system could be defined as patterns of benign activities. In addition, we showed that removing benign activities extracted from a portion of the log data (approximately 1.4% to 3.2% in size) can significantly reduce the search space (up to approximately 52%) in large data sets.

==> declaration.tex <==
\thispagestyle{empty}

%%%
%%% You must sign the declaration of originality. 
%%%
%%% You are submitting this electronically. Therefore, to sign, you 
%%% type your name and date to replace the .... characters. 
%%%
\begin{center}
    {\LARGE\bf Declaration of originality}
\end{center}

I confirm that:

\begin{itemize}
\item{This submission is my own work, except where 
clearly indicated.}

\item{I understand that there are severe penalties for Unacceptable Academic Practice, which can lead to loss of marks or even the withholding of a degree.}
 
\item{I have read the regulations on Unacceptable Academic Practice from the University's Academic Quality and Records Office (AQRO) and the relevant sections of the current Student Handbook of the Department of Computer Science.}
 
\item{In submitting this work I understand and agree to abide by the University's regulations governing these issues.}
\end{itemize}

\vspace{2em}
Name ............................................................  \\

\vspace{1em}
Date ............................................................ \\

%%% 
%%% We would like to make a selection of final reports available to students that take 
%%% this module in future years. To enable us to do this, we require your consent. You 
%%% are not required that you do this, but if you do give your consent, then we will have 
%%% the option to select yours as one of a number of reports as examples for other 
%%% students. If you would like to give your consent, then please include the following 
%%% text and type your name and date to replace the .... characters. 
%%% 
%%% If you do not wish to give your consent, please remove this from your report. 
%%%
\vspace{1em}
\begin{center}
    {\LARGE\bf Consent to share this work}
\end{center}

By including my name below, I hereby agree to this dissertation being made available to other students and academic staff of the Aberystwyth Computer Science Department.  

\vspace{2em}
Name ............................................................  \\

\vspace{1em}
Date ............................................................ \\



